Enhancing Safety of Students with Mobile Air Filtration during School Reopening from COVID-19

The paper discusses how robots enable occupant-safe continuous protection for students when schools reopen. Conventionally, fixed air filters are not used as a key pandemic prevention method for public indoor spaces because they are unable to trap the airborne pathogens in time in the entire room. However, by combining the mobility of a robot with air filtration, the efficacy of cleaning up the air around multiple people is largely increased. A disinfection co-robot prototype is thus developed to provide continuous and occupant-friendly protection to people gathering indoors, specifically for students in a classroom scenario. In a static classroom with students sitting in a grid pattern, the mobile robot is able to serve up to 14 students per cycle while reducing the worst-case pathogen dosage by 20%, and with higher robustness compared to a static filter. The extent of robot protection is optimized by tuning the passing distance and speed, such that a robot is able to serve more people given a threshold of worst-case dosage a person can receive.

==> ICRA - COVID Robot (Version 6663)/classroom.tex <==
\section{Predictive Assessments of Classroom Social Distancing \& Robotic Filtration} 
%\subsection{Modeling for Social Distancing \& Robot Interventions} 
%\subsection{Simulations of Mobile Disinfection Robot}
\label{sec:disinfection_sim}

%PAGE LIMIT: 2.5 PAGES from here to end of references

%As countries transition to the ``reopening phase", maintaining social distancing at 2\,m and wearing facial coverings have become a convention. However, people also tend to relax the facial covering rule over time, with both psychological (getting used to the pandemic and paying less caution) and physical (discomfort induced by the face masks) reasons. Therefore, 
Based on the CFD simulation results, this section assess the risk of virus spreading to the adjacent people. Specifically, the classroom seating model and periodic cleaning model are built, providing parameterized design and optimization approach to efficient robotic air filtration servicing specified number of people.

%The simulations demonstrate sneezing and coughing scenarios and how implementing mobile filtration reduces the risk of exposure compared to standard stationary filtration. Additional experimental work demonstrating the PCPR's efficiency against stationary filters, further demonstrating the reduced exposure to bioaerosols. 


%- Based on the spread model, use a simulation to show how can a mobile robot improve the filtration/disinfection efficiency compared to a fixed unit (Consider simplifying the model obtained in (1) to a Lattice Boltzman Machine of 2-D convection-diffusion, then apply the velocity boundary condition given the source and air filter positions)

\subsection{Modeling of Transmission and Robotic Cleaning of Airborne Pathogen in a Classroom Setting}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/RobotFiltrationPath.pdf}
    \caption{Geometric parameters of the indoor spread and cleaning model. Observers are the people at risk with red asterisks.}
    \label{fig:robot_classroom_cleaning}
\end{figure}

Without losing commonality, occupants (students) are assumed to be static, sitting in a grid with specified and fixed spacing $(d_x, d_y)$, and facing the same ($+d_x$, or right as seen in the figure) direction. As a result, we assume the plume of particles from an emission event does not spread backwards. The virus carrier is unaware of becoming the source of spread, hence the exact source location is unknown. However, when an emission does occur, we identify the five people seated to the front and sides of the source to be the most vulnerable, based on the spreading pattern of the plume as shown in Section \ref{sec:simple_single_source}. These people are denoted as ``observers", whose infection risks of are evaluated with virus dosage as \eqref{eqn:dosage}.

Since robotic filtration works by proactively moving to and cleaning up the plume before it spreads, the robot needs to pass by every occupant in the room to achieve the cleaning task. The reason for cleaning the space near every individual is two folds: only humans can emit the infectious plume, and the virus carrier is randomly hidden among the occupants. For occupants seated in a grid pattern, the simplest pattern of robot motion that 
traverses each occupant is sequentially passing by the front of each row (from left to right of one person, or vice versa) at distance $r\in(0,d_x)$, in a straight line and uniform speed $v$, before turning around to clean the next row, as shown in Fig. \ref{fig:robot_classroom_cleaning}. Compared to moving in column direction, row-directional motion enables the robot to pass in front of each occupant, where the probable concentration of particles is the maximum. We neglect the time the robot spend to switch rows or return after a cycle, because they are relatively fixed depending on the room layout, hence can be added afterwards as overhead. To summarize, the cycle time of the robot, $\tau$ is bounded by the total number of people $N$ the robot is passing:
\begin{equation}
    \tau \equiv NT_1 = Nd_y/v
\end{equation}
where $T_1$ is the service time for each person, further bounded by the lateral spacing of the occupants $d_y$ and the velocity of the robot. We further assume that the robot has a quantum release time, such that if the source emits at $T=0$, the possible times that the robot happens to be in front of the source are $T_C = nT_1, \ \ \ n=0,1,\cdots, N-1.$
Since the robot cleans the room periodically, passing $N$ people has the worst-case latency of $T_{C,\max}=(N-1)T_1$ after the emission from the source.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.49\textwidth]{figures/2src_1stat_fine.png}
%     \caption{The concentration of pathogen at (a) t=1\,s and (b) t=2\,min with TWO static filter at 2\,m from person A, indicated by the magenta '+' mark.}
%     \label{fig:sim_static}
% \end{figure}

\subsection{Optimization of Path Parameters}

The efficacy of the air filtration is defined as the reduction ratio of maximum cumulative dosage per emission event among the five observers, compared to the case without any filtration (i.e. natural precipitation and natural diffusion). Since the exact time of emission is unknown, the objective is set to minimize the maximum dosage for all cleaning delays $T_C$, given a fixed $N$. The parameterized path of the robot left us with two variables to tune -- robot speed $v$ and distance $r$ from each row of people. 
%From the simulation in Section \ref{}, we interpret that the sooner a robot cleans an infectious plume (with higher $v$), the more effective it can suppress the spread. However, the flow rate of the air filter is fixed, which means a higher $v$ will result in lower decrease in concentration per pass. Reducing the distance of the robot from the source can also prevent large area of spread, however it has a tradeoff of more likely missing the plume if $T_C$ is not suitable. 
Therefore, the optimization formula can be expressed as:
\begin{equation}
\begin{array}{l}
    \{v_N^*, r_N^*\} = \underset{v\in(0,v_{\max}), r\in(0,d_x)}{\arg\min} \max\left(\hat{D}_{P_n}(x,y)_{\textnormal{obs}}\right): \\
    (x,y)\in\{(0,\pm d_y), (d_x, 0), (d_x, \pm d_y)\}; P_n\vert_{\forall T_C}
    %, \textnormal{ s.t. }\\ \forall P\vert_{0\le T_C \le(N-1)T_1} :  \hat{D}_P(x,y)_{\textnormal{obs}}\vert_{t_e=1800}<0.625
\end{array}
\end{equation}

%maximizes $N$ with respect to $(v, r)$, such that the maximum particle concentration experienced in the five assessment points still falls within the threshold, when $T_C=(N-1)d_y/v$.

%HOW TO APPROXIMATE THE EFFECT OF AN AIR FILTER PASSING THROUGH THE PLUME AT TIME $T_C$ AND DISTANCE $r$: expanded

Since CFD simulation of exact particle distribution is extremely computationally-intense and time-consuming, it is impossible to perform iterative computation for path optimization of the robotic filter. Therefore, a low-order approximation is developed for the evaluation of the optimization objective. As a preliminary assumption for path parameter optimization, we assume the spread of the plume is not macroscopically affected by the motion of the robot given that the robot is moving slowly. 
%From the CFD results in Section \ref{} we found that the velocity of the plume quickly dissipates after emission, while the diffusion dominates the spread. Therefore, we assume that the robot act as a local reduction ``shader" atop the unperturbed CFD simulation result. Under the ``shader" approximation, if
From Section III-A we identified that the initial momentum of the particles dissipated quickly after emission, therefore the spread can be approximated with a decayed diffusion to extrapolate the CFD data with step size $\Delta t$:
\begin{equation}
    C(x,y,t+\Delta t) = k_t^{\Delta t}\left(C(x,y,t) + k_d \Delta t \cdot \nabla^2 C(x,y,t)\right),
    \label{eqn:diffuse}
\end{equation}
where $C$ is the field to be diffused. $k_d$ is the equivalent diffusivity, and $k_t$ is the time constant of the exponential decay, both estimated using distribution of virus concentration from the CFD results in the time range from 30 to 60 seconds. The estimated values are $k_d \approx 0.003$\,m$^2$/s and $k_t \approx 0.98$, but the actual values depend on the air flow of the room.

During each dosage accumulation time step, the effect of the robotic air filter is simplified by decreasing a factor of $k_f=Q\Delta t/V_r$
on the virus concentration and influx at each discretized grid that is within the footprint of the robot. Here $Q$ is the flow rate of the filter, and $V_r$ is the volume of the column formed by the robot footprint. The decrements are also decayed and diffused using \eqref{eqn:diffuse} before propagating to the next dosage accumulation time step.

%To summarize, the process of estimating the effect of the mobile robotic filter for optimization is:
%\begin{enumerate}
%    \item Set $t=0$, initialize $\Delta_f$ and $\delta_f$ to be zero matrices;
%    \item Interpolating two adjacent CFD results to obtain the time difference $\Delta C_0$ of the unperturbed distribution of virus concentration $C_0$;
%    \item Compute the pre-filter concentration $C_f = C_0 - \Delta_f$ and time difference $\Delta C_f = \Delta C_0 \odot (1-\delta_f)$, where $\odot$ denotes the element-wise multiplication;
%    \item Perturb with the filter by multiplying $C_f$ and $\Delta C_f$ at grids within $V_r$ by $(1-k_f)$;
%    \item If CFD results at future times are \textbf{not} available, diffuse $C_f$ with \eqref{eqn:diffuse} and goto Step 9)
%    \item Compute $C_0\leftarrow C_0+\Delta C_0; \ \ C_f \leftarrow C_f + \Delta C_f$
%    \item Compute the difference caused by the filter $\Delta_f \leftarrow C_0 - C_f$ and the reduction ratio $\delta_f \leftarrow \Delta_f \odot (1/C_0)$
%    \item Diffuse $\Delta_f$ with \eqref{eqn:diffuse}
%    \item Compute dosage with \eqref{eqn:dosage}.
%    \item Set $t\leftarrow t+\Delta t$. If CFD results at future times are available goto Step 2), else goto Step 4) and set $\Delta C_f = 0$.
%\end{enumerate}

The dosage evaluation ranges from 0 to 600\,s for convergence, and uses a step size of 1\,s. The evaluation is implemented in MATLAB with the optimization process realized through the \texttt{fmincon} function. CFD result from a single source is referred to in the time range of 0 to 60\,s, as the velocity of the plume after 60\,s is small and therefore susceptible to perturbations. 
The optimization results show that the efficacy of the robot, with a given $N$, increases with $r$ and $v$. The efficacy of the robot decreases monotonically with the increase of cleaning cycle $\tau$, i.e. the number of people $N$ it is passing. However, with large passing distance the cleaning delay $T_C$ becomes less sensitive. The optimization result also show that among the five observers, the one in the Front Center position is the most vulnerable, in that it receives the highest dosage.

The projected cumulative dosage per emission for the Front Center position, under different passing distance and velocities, is shown in Fig. \ref{fig:slices}. An experiment is carried out to validate the optimization result in real-world indoor airflow, and using a mimicked source.

\begin{figure}
    \centering
    \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1.0\linewidth, trim = {0 0 0 5mm}]{figures/DosageVSSpeed.pdf}
    \caption{Dosage vs. Speed, \\assume passing at $r=1.3$\,m.}
    \end{subfigure}
    \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1.0\linewidth, trim = {0 0 0 5mm}]{figures/DosageVSDistance.pdf}
    \caption{Dosage vs. Passing Distance, \\assume passing at $v=0.5$\,m/s.}
    \end{subfigure}
    \caption{Projected trend of cumulative dosage with a robotic filter during a single cough event, at Front Center point, with respect to design parameters and people serviced.}
    \label{fig:slices}
\end{figure}

==> ICRA - COVID Robot (Version 6663)/conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}

The Purdue Campus Patrol Robot combines mobility in robots with air filtration, which achieves effective, robust, and occupant-friendly cleaning of classrooms. The robot, capable of serving more than 10 students at once, effectively reduces worst-case dosage that a people can receive in case of a cough in a classroom. As a result, the safety of students can be further enhanced while sporadic outbreak further prevented during school reopening from COVID-19. The workflow of modeling and optimization provides insights to future design of the robot and arrangement of robot-friendly classrooms.

==> ICRA - COVID Robot (Version 6663)/experiment.tex <==
\section{Experimental Validation on the Efficacy of Robotic Mobile Air Filtration}
\label{sec:exp}

%[TODO: CHANGE THE SOURCE TO AN INFLATED BALOON]

%[TODO: MEASURE CONCENTRATION IN MULTIPLE POINTS IN THE ROOM]

%[TODO: CONSIDER USING A LAB / CLASSROOM]

Although optimizations in \ref{sec:disinfection_sim} showed promising results that the robot is able to reduce the dosage received by the people closest to the source, the real-world airflow may affect the results drastically. As a validation, we carried out an experiment, physically duplicating the case in Fig. \ref{fig:robot_classroom_cleaning} in a realistic indoor environment.

\begin{figure}
    \centering
    \includegraphics[width=0.81\linewidth]{figures/RobotExp.pdf}
    \caption{Experiment with PCPR and a mimicked source. The airfoils of the Bernoulli Air Filter were removed to match the simulation and optimization assumptions. The red arrows indicate the robot's cleaning and return paths.}
    \label{fig:expSetup}
\end{figure}
As shown in Fig. \ref{fig:expSetup}, we align chairs in a room of 5\,m$\times$6\,m, following social distancing guidelines at Purdue, with $d_x=2.0$\,m and $d_y=1.5$\,m. We assume the center seat at the rear is the source, and five article counters (ExTech VPC300) are placed at the observer (Front Left, Front Center, Front Right, Left, and Right) locations. Since the magnitude of emission velocity affects spreading speed of the plume, hence affects the cleaning efficacy of the robot, the horizontal velocity of the emission should match that of a normal human cough as discussed in Section \ref{sec:simple_single_source}. The number of particles emitted, however, can be scaled up to obtain better signal to noise ratio over the background particle counts.

In the experiment we use a vector fogger with pitch-up angle of 65$^{\circ}$ and copper mesh at the nozzle to obtain a peak horizontal speed of 22\,m/s. 
%The copper mesh reduces the average outlet speed from 30\,m/s to 26.8\,m/s, while the 65$^{\circ}$ pitch angle creates a horizontal component of 11.3\,m/s, which equals to the conditions set in the simulations (average speed equals to one half the maximum speed of 22.06\,m/s). 
A plastic bag loosely covers around the nozzle and the mesh to collect the backflow and the droplets within. The source was turned on for 2\,s each, and the measurements at the five observers last for 10 minutes. The particle counter reads the accumulative counts for particles of diameters 0.3, 0.5, 1.0, 2.5, 5.0, and 10\,$\mu$m, hence the total 10-minute dosage based on volume of inhaled particles can be calculated with \eqref{eqn:dosage}. The background is measured and subtracted prior to the start of each cumulative measurement series. Since the number of particles is scaled up compared to a normal human cough, we compare the relative dosage by scaling the highest value observed down to 1.

Following the guidelines obtained from Section \ref{sec:disinfection_sim}, we set the passing distance of the robot to be $r=1.3$\,m, which is the maximum distance without the robot hitting the legs of the chairs in the front row. The speed of the robot moving through the cleaning zone (i.e. between the two rows) is set to be $v=0.5$\,m/s. After completing each pass, the robot moves out of the cleaning zone and circulates back to the starting point within specified time. The circulation behavior simulates the cleaning of other spaces, with the cycle time set to $\tau=30$s, $36$s, and $42$s, corresponding to $N=10, 12, 14$, respectively. The source is released such that the cleaning delay $T_C = \tau-3$,  the maximum cleaning delay possible. Three additional cases are set up as comparisons: A) ``Near Static Filter": the static filter is placed at 1.3\,m in front of the source; B) ``Far Static Filter": the static filter is placed 2\,m in front of the Front Center person, simulating a centralized filter placed at the center of a larger room; C) no air filtration is provided.

The normalized dosages at the five observers in different cases are shown in Fig. \ref{fig:dosage_compare}. From the results we conclude that our robot setup is able to decrease the dosage that people around the emission source receive by at least 20\% when servicing 14 people, which is the capacity of an average classroom when social distancing guidelines are observed. The cumulative dosage slightly decreased as $N$ goes from 10 to 14, which as we interpret, is due to increased background that drowns out the tail of the dosage accumulation, as these experiments happens in chronological order. The experimental result outperforms that obtained from the optimization simulation, and the dosage distribution among the five observers are not always symmetric, which we discuss as follows:

\begin{figure}
    \centering
    \includegraphics[width = 0.95\linewidth]{figures/all.pdf}
    \caption{Cumulative dosage comparison of the five assessment locations under different filtration settings.}
    \label{fig:dosage_compare}
\end{figure}

\subsubsection{Wake of the robot attracts particles to boost cleaning effects}
The motion of the robot creates a low-pressure zone behind the robot that traps particles along with the robot. The effect was seen through CFD simulation as well. The wake, as a bonus from mobility, improves cleaning efficacy while also poses design considerations on the shape of the robot. The airfoils of the Bernoulli filter is an example that utilizes the wake to keep stable traction to the particles as the robot moves.

\subsubsection{Volatility of indoor airflow}
Some of the experiment results show biased dosage distribution to the right, which is due to the design of air conditioning system in the room. The volatility of indoor airflow also demonstrated the robustness of the robotic filter, compared to the Near Static Filter case, in cleaning particles that deviated from their theoretical positions.

\subsubsection{Considerations on classroom arrangements} In order to utilize the $N$ most effectively, for robotic filtration, classrooms should be arranged in the lateral direction to reduce row switching time for the robot.

\subsubsection{Real-time environment assessment for pathogens to optimize cleaning efficiency} PCPR seeks to integrate biosensors for pathogen detection, which in real time assess the robot surroundings. The real-time environment information will be invaluable to dynamic planning and optimizing the efficiency of air and surface disinfection,

==> ICRA - COVID Robot (Version 6663)/intro.tex <==
\section{Introduction}

Robots were initially proposed as a protective measure for healthcare workers during the the Ebola outbreak in 2014 \cite{Kraft2016RobotForInfectiousDiseases, robotEbola2014Assessment} -- by performing risky but low-skill tasks such as cleaning.
%-- by assisting in frequently-practiced low-skill tasks such as cleaning, waste management, and logistics, to reduce hospital worker exposure -- instead of replacing the medical workers completely. 
%However, its application during the Ebola pandemic was limited because of the social, geological, and technological constraints -- the epicenter was localized in west Africa and electricity, communication, and public knowledge were unable to support grounded adoptions of robots.
%\subsection{What's different and what's the same?}
During the COVID-19 pandemic, the urban infrastructure of the hot-spots enable wider and more effective use of robots -- from aerial to ground robots -- to enhance people's safety and reduce the spread \cite{2020RobotsForInfectiousDiseases}. Among them, clinical care robots emerged mostly during the \textit{onset phase} of COVID-19, as in prior pandemics. They were superceded by robots for public safety as the pandemic spreads and policies evolve into \textit{quarantine phase}. Finally, as we enter the \textit{reopening phase}, robots for workplaces and schools become significant. %Finally, as we enter the reopening phase robots for workspaces and schools srobots concerning work and education rises significantly dauring \textit{reopening phase} as schools and businesses prepare for restart.

%Our research team has been following this trend from medical-specific to general public applications, specificaly on how robots can protect students and essential workers that are under risk of virus exposure during the reopening of the economy. 
%To address widespread PPE shortages among healthcare workers during \textit{onset phase}, we initially developed the teleoperated Tsinghua Clinical Patrol Robot (TCPR) to remove healthcare workers from close-contact screening tasks. As time progresses, the demand for general protection shifts to essential workers such as retail staffs during the \textit{quarantine phase}, and further to the major public during the \textit{reopening phase}. The shift in demographics of people susceptible to work exposure accordingly changes the type of robotic functions required to protect them. Consequently, a second robot prototype, 
As PPE supplies catches up and eases pressure on medical staff, community spread becomes the focus of suppressing and reopening from the pandemic. While the exposure rate to virus is low in non-hospital facilities, the risk is accumulated by the long exposure time and number of people involved. Therefore, the necessity lies in preparing educators and essential workers to safely move within suddenly hazardous environments. Driven by these requirements, the Purdue Campus Patrol Robot (PCPR) is developed (Fig. \ref{fig:robot}) to protect people in indoor public places using multimodal disinfection. Among which, the occupant-friendly robotic air filtration fills an urgent need as schools reopen and gatherings in classrooms pose dangerous spreading occasions of the virus through bioaerosol created when sneezing, coughing, or even breathing.

\begin{figure}
    \begin{subfigure}{0.7\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth, trim={0 10mm 0 4mm}]{figures/OmniveyorFullSetup.pdf}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.28\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth, trim={75mm 0 0 0}, clip]{figures/robotpic.jpg}
    \caption{}
    \end{subfigure}
    \caption{The Purdue Campus Patrol Robot (PCPR). (a) The overall assembly and effective disinfection payloads; (b) A physical figure of the robot showing the setup of the Bernoulli Air Filtration Module.}
    \label{fig:robot}
\end{figure}

%[ADD LITERATURE REVIEW ON MOBILE DISINFECTION]
Previous literature featuring robot for disinfection involves either chemical spraying \cite{s20123543SprayRobot, 6840192WallCleaningRobot}, or ultraviolet (UV) light exposure \cite{YANG2019487UVC, RobotInContagiousWorld}. While these methods kills the pathogens directly and are also involved in our robot design, they poses irritation to people around it, hence they are not suitable for full-time protection of indoor personnel. Conventionally, stationary air filtration systems alone is not effective for epidemic prevention \cite{Lee_2011_BioaerosolControl}, because the pathogen may find its victim before being circulated to and trapped by the filtration system. On the other hand, the effect of combining an air filtration system with a moving robot has not been studied before. 
This paper shows that the mobility of robots augments air filtration to achieve well-covered protection of indoor people against scattered sources of airborne pathogen. 

As an overview, the contributions of this paper are:
\begin{itemize}
    \item Designed and built the Purdue Campus Patrol Robot -- a prototype for indoor mobile air filtration, which promotes effective, continuous and occupant-friendly protection in a classroom setting.
    \item Proposes a class of parameterized trajectory in a robot-friendly classroom arrangement, and optimizes the parameter to minimize the infection risk of people adjacent to the source, given the total number of people the robot is servicing.
\end{itemize}

The remainder of the paper is organized as follows: Section \ref{sec:odr} gives an overview of the urgency of the problem and the PCPR setup. The spreading dynamics of bioaerosol and the risks involved is further analyzed in Section \ref{sec:simple_single_source} with numerical simulation. Section \ref{sec:disinfection_sim} builds a generalizable model of virus spreading in classrooms, where the efficacy of our robot is analyzed and optimized. Section \ref{sec:exp} compares the optimization results with that obtained in an experiment using a mimicked source. Finally, Section \ref{sec:conclusion} draws the conclusion.

==> ICRA - COVID Robot (Version 6663)/robot.tex <==
\section{Overview of the Purdue Campus Patrol Robot for Mobile Disinfection}
\label{sec:odr}

The PCPR (Purdue Campus Patrol Robot) 
%evolved from the TCPR prototype to 
integrates robotics into indoor public settings tasked to carry out repetitive and occupant-safe disinfection procedures. 
Due to the covert and contagious nature of the virus, symptom-less people still pose risk of spreading the virus to the susceptible, posing persistent pressure to sporadic outbreaks. Therefore, well-covered, efficient disinfection when people are gathering indoors is essential to suppressing community spread. 
%With the pandemic passing its peak, the economy begins to push forward into the \textit{reopening phase}, despite the persisting pressure of scattered outbreaks due to the covert and contagious nature of the virus. Analogous to the quarantine phase, the risk of infection accumulates with prolonged exposure time, hence the PCPR can still protect the susceptible people through well-covered, efficient disinfection.
%The effectiveness of employing automated disinfection measures in community environments was tested using common cleaning techniques such as air filtration, ultraviolet (UV) light, and liquid disinfectant.
%UVC light of the intensity necessary to kill viruses at these distances is not considered human safe, so it is only suitable for retail operations overnight, when customers are not present. Furthermore, it requires long ``exposure times" to effectively kill viruses and also requires careful room preparation at the precise time that is often most dangerous to employees. For these reasons, it is not appropriate for isolation of retail workers when customers are present.
%Disinfection methods in public spaces involve employing ultraviolet (UV) light in the UVC band, and chemical spraying. However, UVC light is not human safe, and chemical spraying currently depends on human workers which exposes them to the virus. 
Specifically, the classroom scenario serves as a simple but typical model for the types of disinfection during the \textit{reopening phase}. The people are statically located while obeying social distancing, while the transmission through both bioaerosol and contact of contaminated surfaces exist. The variety of transmission paths require a variety of complementary capabilities of periodical and effective disinfection during hours of operation. 

\subsection{Problem Statement}

Schools have been taking measures in arrangement to prevent community spreads during reopening. For example, Purdue University mandated seating spacing in classrooms of 2 meters longitudinally and 1.5 meters laterally. Some classrooms have additional fans set up at the doors for ventilation. However, the social distancing guidelines are based on either emperical guess or over-simplified assumptions, which may result to failure in protection \cite{Setti2020-6ftNotEnough}. As static air filtration and venting methods become an assistive measure to keep the indoor pathogen concentration low, they have coverage issues -- the source can be in any possible locations in the room, which means ideal airflow to vent or clean the pathogens is not guaranteed. On the other hand, placing an air filter in front of every occupant in the room is costly and not feasible when the number of occupants scale. Therefore, we are interested in how robots can suppress the spread by combining mobility with air filtration.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/SimpleTraj.pdf}
    \caption{A simple trajectory of the robot when cleaning a space with four people}
    \label{fig:sim_rob_path}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{1.0\linewidth}
        \includegraphics[width = 1.0\linewidth, trim={5mm 35mm 12mm 35mm}, clip]{figures/Robot60.pdf}
        \caption{Robotic Filter Case}
    \end{subfigure}
    \begin{subfigure}{1.0\linewidth}
        \includegraphics[width=1.0\linewidth, trim={6mm 35mm 10mm 35mm}, clip]{figures/Static60.pdf}
        \caption{Static Filter Case}
    \end{subfigure}
    \caption{Saliva droplet distribution comparison at 1 minute after emission from two simulated coughing sources.}
    \label{fig:sim_robot}
\end{figure}

A simple comparative simulation is set up as Fig. \ref{fig:sim_rob_path} to illustrate the problem more intuitively: 4 people (A, B, C, and D) are placed in a room of 3\,m$\times$8\,m with coordinates as specified to follow social distancing guidelines, and all people faces to the right. In one case, a static filter is set at the geometric center to ensure least sum of distances to the four people, while in another case, the same filter is placed on a mobile robotic base that moves cyclically on the specified path across the middle points between people, with a specified velocity of $v=0.5$\,m/s. Since every person can possibly be the source, we specifically make persons A and C be the source of virus and they cough simultaneously. We evaluate the spreading pattern in the two cases using Computational Fluid Dynamics (CFD) simulation, which will be elaborated in Sec. \ref{sec:simple_single_source}. The distribution of particles after 1 minute, in both cases, are compared side by side in Fig. \ref{fig:sim_robot}, which clearly shows the advantage of the robotic filter over the static filter in cleaning speed and coverage. For persons B and D, slower cleaning of the plume means longer and faster accumulation of their dosages of the virus, hence poses higher risks of infection. The simple simulation signifies the improvements of a mobile robotic filter over a static filter, when multiple people are in the room without proper ventilation.

%\subsubsection{Design Considerations for PCPR} %{Design Cnsiderations Based on Lessons Learned} %

%We need to link this better to the Tsinghua robot and lessons learned. why design this? Don't need to focus on the OmniVeyor base design

%Considerations:

%Backseat driving that can be taken over at any time;

%Handling devices not designed for robots;

%Communication: teleoperation with low bandwidth requirements;

%Path planning driven by disinfection doses and plume models.

%robot not becoming the source of spread : robot PPE
 
%robot hides away harmful rays and chemicals from human operators : design of air filtration systems, sprays, remote operation
 
%robot are more effective at disinfecting than fixed units

%Design:
    
% - About the Omniveyor (robot base);

%The TCPR prototype covered the manipulative forms of disinfection via teleoperation, so the PCPR prototype focuses on non-manipulative forms of disinfection. As a result, the robot
\subsection{Robot Composition}

The PCPR consists of three main parts: a holonomic mobile base, a spraying system, and an air filtration unit with internal UV disinfection. The omnidirectional holonomic base handles the navigation and obstacle avoidance with a planar LiDAR and two RealSense cameras. Its capability of holonomic motion eases constraints on path planning for directional payloads such as air filtration unit. Core safety techniques for collision avoidance are inbuilt to the base, ensuring the robot stops and circles around if it gets too close to any obstacle. With three parts combined, the robot can effectively perform autonomous multimodal disinfection on air and surfaces in an indoor space.

%The latter demonstrates, through simulation, the efficacy of robotic air filtration for reducing exposure of workers and customers to the SARS-CoV-2 virus as compared to stationary techniques. It also provides a prescriptive tool for administrators to plan for social distancing and robotic disinfection in education and retail contexts. 

%Horizontal modes of transmission of SARS-CoV-2 involve droplets, bioaerosols, and indirect infection through shared objects/surfaces. To reduce essential worker exposure to horizontal transmission, the robot serves as an assistant to actively disinfect community spaces in place of essential workers. Unlike standard disinfection systems (stationary air filtration systems and handheld/backpack spraying systems), the robot is more effective on containing discrete emissions of pathogens, while hiding people away from harmful exposures to disinfectants, UV light, and the pathogen itself.

%Therefore, the robot acts as a safeguard---i.e., an environmental disinfector---to block virus transmission for service workers. The robot is designed to eliminate pathogens spread through air and surface, as the two significant spread media of COVID-19. 

%For maneuvering the disinfection payload, the robot consists of an omnidirectional mobile base with 4 powered caster wheels driven by 8 motors \cite{Holmberg2000PoweredCaster}. The robotic base uses a standard navigation stack, with odometer and LiDAR sensors, to support autonomous map navigation and dynamic obstacle avoidance. 
%An operational space controller handles the overactuated mechanism, generates desired motion of the robot with decoupled three degrees of freedom, and outputs the odometry information as a byproduct. 
%The robot's omnidirectional holonomic motion capability eases the constraints on trajectory planning for directional disinfection payloads. 
%For example, the decoupling of steering and movement enables the robot to rotate while moving towards the desired direction, providing 360 degrees of coverage for directional air intake of the air filter.

%The mobile base handles navigation and obstacle avoidance while operating through the working spaces. The objective of the path planning is to cover the whole working area with the effective radius of its on-board disinfection payload while addressing droplet and aerosol transmission by coughs or sneezes. The mobile base involves a standard navigation stack that consists of an odometer and a 2-D LiDAR. A 2-D map of the workspace was initially given to the robot, based on which the localization was established using the LiDAR and odometer, with adaptive Monte-Carlo method \cite{}. The obstacle avoidance is achieved using timed elastic band method \cite{}, such that deviation from desired travel time between via-points is minimized even at the presence of obstacles, which is critical to ensuring the desired accumulative dosage. 
%Additional information of the obstacles is provided by the RealSense cameras, such that persons can be identified and protected / targeted.

%Unlike the expertise required of doctors for robot-assisted medical care, robotic disinfection requires less practice with the robot for users to be effective. %However, the same applies as reduced trust in a fully autonomous robot to carry out safety considerations. To alleviate these concerns, 
%To accommodate user friendliness and other feedback from TCPR trials, 

%The PCPR prototype is designed for ``remote backseat driving" to account for scalability in deployment and coordination between robots for high coverage efficiency. Effectively, this is a ``robot call center" that allows the robot to request a remote trained operator to safely get the robot unstuck from difficult, unforeseen situations (such as crossing a narrow doorway) using live feedback from the cameras. Then the escape strategy used by the remote operator is encoded into the cache of error correction strategies.

%Additionally, using a remote center to control multiple robots enables coordination in a batch deployment to achieve high coverage efficiency.
%These measures reduce the perceived lack of trust in such fully autonomous robots.  

% this is not especially necessary since this is defined in later sections. -- To summarize, the disinfection robot consists of an electrostatic micro-spray dispenser and an air filtration system with UVC disinfection, mounted on a mobile robotic base. The robot is covered with anti-microbial coating that mitigates the spread of the contamination. Each component will be explained in further detail as follows, and concludes with a validation of its effectiveness compared to a fixed unit using both simulation and experiments.

The remainder of this section describes the two forms of non-contact disinfection that the robot is capable of performing -- disinfectant spraying and mobile air filtration, among which mobile air filtration is novel. The spraying module has a static coverage radius, while the coverage dynamics of the air filtration system is not obvious. Hence, the analysis on the efficacy of air filtration will be expanded in Section \ref{sec:disinfection_sim}.

%\subsection{Nanoparticle Coating as Robot PPE}

%PPE cannot be limited to professional medical practitioners by teleoperation, but also shall cover all vulnerable essential workers on site by means of effective disinfection.

%Effective measures for reducing virus transmission to essential workers necessitates implementing contactless disinfection measures.
%The robot moves through high-risk areas as a substitute of essential personnel to carry out disinfection procedures. While major paths of horizontal transmission---through inhaling contaminated air and directly touching contaminated surfaces---will be eliminated, however, a small chance of transmission still exists. That is the robot being contaminated by the working environment. Since the virus normally is carried by micro-droplets of saliva, the robot is equipped with a conjugate hydrophobic and lipophobic coating to repel pathogens to preventing itself from becoming a source of spread. The coating composes of lasting nanoparticles of an inorganic broad spectrum photocatalytic disinfectant, which inactivates 99.9\% of bacteria and viruses that are picked up over the course of the cleaning process.
%By replacing the humans with robots, one major benefit in the dynamics of infectious diseases is that the robots don't breathe and don't host the pathogen (i.e. the pathogen can not multiply on the inorganic robot), thus it will not actively disperse the disease. However, for infectious diseases transmitting through both contact and respiration, the robot 
%replacing human workers in 
%automating some of the disinfection tasks, it 
%could potentially become a media of transmission by being contaminated by the infected. Thus, analogous to PPE for humans, robot should be covered with robot PPE, i.e. a protective coating which eliminate or reduce transmission via the robot surface. 

 
%For the developed disinfection robot, this is achieved by using protective nanoparticle coating which kills all viruses from the surface of the robot. 
%Nanoparticle coatings have a much greater surface area per unit mass compared with the larger particles, making them more reactive. 
%A broad spectrum, inorganic nanoparticle-based disinfectant [NEEDS CITATION], is used as both the coating material and disinfectant spray. This coating breaks the surface of bacteria, viruses, and fungi and inactivates them using a photocatalytic process to which they cannot generate resistance. Laboratory tests validate that this coating eliminates 99.9\% of the microorganisms. The nanoparticle coaing will remain active on the robot's surface as long as the pathogens are not eliminated from the target location. It can be applied to a wide range of surfaces such as metal, wood, fabric, plastic and ceramics for disinfection. 

% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/nanoxen.png}
% 	\caption{Nano-based photocatalytic process of pathogen killing }
% 	\label{fig:nanoxen}
% \end{figure}

\subsubsection{Disinfecting Spray Module}

Spraying disinfectants is a hospital-proven measure of epidemic prevention \cite{otter2013role}. %, and is currently used on public benches, shopping carts, aisles and storage shelves. 
However, it is a labor-intensive job performed by staffs, % with handheld or backpack sprayers.
who are exposed to two-fold hazard risks without extensive protection -- disinfectants usually cause irritation to human body, and the contaminated surfaces poses risks of infections. The spraying system on the robot uses a novel nanoparticle disinfectant solution and micro-spray system that can run either pre-scheduled or teleoperated, which removes staffs from the harsh working environment. 
The spray module has nozzles on both sides and rear of the robot, since spraying from the frontal side interferes with the perception sensors. The nozzles produce a cone-shaped micro-droplet cloud of disinfectant with an average droplets size of $\sim50\,\mu$m, covering a radius of up to 2.25\,m from the robot. An optional Electrostatic Spray Deposition (ESD) sprayer can be added to enhance coverage in corners and hard-to-reach areas.

\subsubsection{Novel Bernoulli Air Filtration Module}

Infectious bioaerosol droplets with diameters ranging from 0.1 to 10\,$\mu$m, which can suspend in air for hours, pose a major threat for horizontal transmission through inhalation.
The PCPR employs a novel air filtration module to increase the effectiveness of robotic filtration. The Bernoulli air filtration module brings medical-grade air treatment---a combination of particle filtration (a High Efficiency Particulate Air (HEPA) filter) and UV disinfection---to public indoor spaces, aiming to inactivate infectious bioaerosol droplets.

%Following the 2003 SARS outbreak, implementing various bioaerosol protocols to protect healthcare workers became of the utmost importance. Infectious bioaerosol droplet size ranges from 0.1 to 10\,$\mu$m, which can remain suspended in the ambient environment for several hours \cite{tsai2006airborne} and can be inhaled by humans. Hospitals are equipped with extensive measures to mitigate bioaerosols using various air filtration systems, but public and community settings are seldom equipped with medical-grade filtration systems. The Bernoulli section mounted on the robotic mobile base moves through high-traffic public areas to continuously filter the air ensuring essential worker safety.

In our setup, the filtration efficiency, measured in percentage of the captured particles, is higher than 99.3\% for particles larger than 0.3\,$\mu$m, with capacity of 47\,L/s air. In the cylindrical air duct of the Bernoulli filter, two germicidal 2.5\,W UV lamps with surfaces irradiation of 5\,mW/cm$^2$ are adopted. Being contained inside the cylinder, the UV light poses no exposure risk to passersby.

%\begin{table}[]
%\begin{center}
%\caption{Number of particles with different sizes measured at the inlet and outlet of the air filtration system.}
%\label{tab:airFilter}
%\begin{tabular}{ | m{5em} | m{1.5cm}| m{1.5cm} |  m{1.5cm} | } 
%\hline
%Particle size& Particles at inlet & Particles at outlet & Efficiency\\ 
%\hline
%0.3 $\mu$m & 4620 & 32  & $\sim$99.3\% \\ 
%\hline
%0.5 $\mu$m & 1645 & 0 & $\sim$100\% \\ 
%\hline
%1.0 $\mu$m & 174 & 0 & $\sim$100\% \\ 
%\hline
%2.5 $\mu$m & 29 & 0 & $\sim$100\% \\ 
%\hline
%5.0 $\mu$m & 6 & 0 & $\sim$100\% \\ 
%\hline
%10.0 $\mu$m & 3 & 0 & $\sim$100\% \\ 
%\hline
%\end{tabular}
%\end{center}
%\end{table}

The flow tract design of the Bernoulli module, i.e. the AeroMINE\texttrademark (Motionless, INtegrated Extraction) technology, originates from wind energy applications \cite{houchens2019novel}. Using a pair of mirrored perforated airfoils and a perforated cylindrical tower, 
a low pressure zone is created between the airfoils which helps to drive the air from surroundings into the intake of the system, which then will be driven by an axial fan in the cylinder through an filter. This design achieves large intake area without using a large-diameter fan, thus improves energy efficiency.  
The large intake area creates a large swept volume to trap the pathogen as the robot moves, which is ideal for robotic disinfection.  %The design and the validation of the Bernoulli module were achivied via computational fluid dynamic (CFD) simulations by optimizing the airfoil shape, size, and geometrical modifications to its design.


==> ICRA - COVID Robot (Version 6663)/simulation-simple.tex <==
\section{Transmission Pattern of Airborne Pathogen and Dosage Assessment}
\label{sec:simple_single_source}

%Intuitively introduce the one and two source case.

To investigate the transport and dispersion of saliva droplets in an indoor environment and cast insight on how robots can help, CFD simulations of a single coughing source were performed. Based on which, we extracted the evaluation metrics to differentiate the robotic filter versus a conventional stationary filter, and created snapshots for estimating the effects of a robotic filter.

\subsection{CFD Simulation Setup for Single Coughing Source}\label{sec:cough_snz_model}

Respiratory pathogens can be emitted in the form of bioaerosol when an infected person sneeze, cough, or even breathe. Specifically, we are interested in the coughing case since it is more covert and frequent compared to sneezing, while having similar emission magnitude (in terms of jet velocity) in some conditions \cite{Tang2013SneezeCoughVel}. We also consider a worst-case scenario when no facial coverings is present, as people tend to relax caution on the rules over time. The results from the CFD simulation provide building blocks for optimizations afterwards, and to show that 2\,m (6\,ft) of social distancing is not always sufficient.

With ANSYS Fluent 2019, the room geometry is built as a rectangular domain of 3\,m $\times$ 8\,m $\times$ 3.5\,m (width $\times$ length $\times$ height). 
%Consider a closed room environment with an infected person at one end of the room. Here we evaluate the exposure of another person to saliva droplets, when the infected person coughs and sneezes, through CFD simulations using ANSYS Fluent 2019. The room geometry is built as a rectangular domain of 3\,m $\times$ 8\,m $\times$ 3.5\,m (width $\times$ length $\times$ height) with a small cylinder of 21\,mm that represents an average human mouth \cite{gupta2009flow} located at 1.70m from the floor. The computational domain was discretized into 68000 elements with polyhedral elements.%, as is shown in Fig. \ref{fig:domain} .
%[Keep this for technical reference for now.]
For simulating the turbulent airflow of coughing cases, the Reynolds Average Navier-Stokes (RANS) with the Renormalization Group (RNG) $k$-$\varepsilon$ turbulence model was used in the simulations for its accuracy, computing efficiency, and robustness \cite{hang2014influence}. 
The Lagrangian method was used to track saliva droplets with hybrid implicit and trapezoidal schemes. To emulate a real human cough, saliva droplets are ejected from the mouth with velocity profiles based on previously performed measurements \cite{gupta2009flow, aliabadi2010cfd}. In our case, 14000 droplets with diameters ranging from $2r_P$ = 1\,$\mu$m to 500\,$\mu$m and following Rosin-Rammler distribution \cite{Lindsley2012CoughParticle}, were injected from the inlet for the coughing event. The coughing jet lasts 0.61\,s with a peak velocity around 22.06\,m/s occurring at 0.066\,s. 
%, and the sneezing puff lasts 0.61\,s with a sneeze peak velocity around 89.90\,m/s occurring at 0.1\,s. 
%The transport equations for the two-equation RNG $k$-$\varepsilon$ turbulence model are given as:
%\begin{equation}
%\scalebox{1.0}{$
%\frac{\partial}{\partial t}(\rho k) + \frac{\partial}{\partial x_{i}}(\rho k U_{i})=\frac{\partial}{\partial x_{j}}(\alpha_{k} \mu_{t} \frac{\partial k}{\partial x_{j}})+G_{k}+G_{b}-\rho\varepsilon $}
%\end{equation}
%and
%\begin{equation}
%\scalebox{0.9}{$
%\frac{\partial}{\partial t}(\rho \varepsilon) + \frac{\partial}{\partial x_{i}}(\rho \varepsilon U_{i})=\frac{\partial}{\partial x_{j}}(\alpha_{\varepsilon} \mu_{t} \frac{\partial \varepsilon}{\partial x_{j}})+C_{1 \varepsilon}\frac{\varepsilon}{k}G_{k}-C_{2 \varepsilon}\frac{\varepsilon^2}{k}\rho-R_{\varepsilon}
%$}
%\end{equation}

%Where $\alpha_{k}$ and $\alpha_{\varepsilon}$ are the inverse effective Prandtl numbers for $k$ and $\epsilon$, respectively. $G_b$ is the generation of turbulence kinetic energy due to buoyancy, $G_k$ represents the generation of turbulence kinetic energy due to the mean velocity gradients. The constants $C_{1\epsilon}$ and $C_{2\epsilon}$ derived analytically by the RNG theory \cite{orszag1993renormalisation} have values of 1.42 and 1.68, respectively. The turbulent viscosity $\mu_{t}$ is given by:

%\begin{equation}
%\mu_{t} = \rho C_\mu \frac{k^2}{\epsilon}
%\end{equation}


%With a constant value $C_{\mu} = 0.0845$, derived using RNG theory. The $R_{\varepsilon}$ term in the the RNG $k$-$\varepsilon$ model is the main difference with the standard $k$- $\epsilon$ model. this term significantly improves the accuracy for rapidly strained flows \cite{fluent2013ansys}\cite{escue2010comparison}.The $R_{\varepsilon}$ term given by:

%\begin{equation}
%R_{\epsilon} = \frac{C_\mu \rho \eta^3 (1-\eta/\eta_0)}{1+\beta\eta^3} \frac{\epsilon^2}{k}
%\end{equation}
%where,
%\begin{equation}
%\eta \equiv Sk/\epsilon, \ \ \eta_0 = 4.38, \ \ \beta = 0.012
%\end{equation}

% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/Domain.png}
% 	\caption{Mesh and computational domain calm indoor environment}
% 	\label{fig:domain}
% \end{figure}

%The ambient conditions in the room are modeled after typical indoor spaces (21.5$^{\circ}$C, 50\%RH). All walls were treated as adiabatic with the non-slip wall condition, and a constant value of 0\,Pa was imposed on the pressure outlet. % The velocity–pressure coupling parameter was handled with the SIMPLE method. The PRESTO! (PREssure STaggering Option) scheme were used for the pressure discretization, and for the space discretization a second order upwind scheme was used for the convective terms in the governing equation. 

% of 0.001s up to 1s, 0.01s up to 10s, and 0.1s up to 10 min were used. 

%Fig. \ref{fig:IEEE_cough_streamwise} shows the droplet distribution for the coughing case at 0.5\,s and at 5\,min. Similarly, Fig. \ref{fig:IEEE_sneez_streamwise} shows the droplet distribution for the sneezing case at 0.5\,s and 5\,min.

% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=1\linewidth, trim={10mm 20mm 23mm 20mm}, clip]{figures/SneezeCFD.pdf}
% 	\caption{Computational domain geometry and its inlet velocty profiles emulating sneezing and coughing.}
% 	\label{fig:sim_single_source}
% \end{figure}


% \begin{figure}[htbp]
% \begin{subfigure}{1.0\linewidth}
% 	\centering
% 	\includegraphics[width=1\textwidth]{figures/coughing.pdf}
% 	\caption{Coughing}
% 	\label{fig:IEEE_cough_streamwise}
% 	\end{subfigure}
% \begin{subfigure}{1.0\linewidth}
% 	\centering
% 	\includegraphics[width=1\textwidth]{figures/sneezing.pdf}
% 	\caption{Sneezing}
% 	\label{fig:IEEE_sneez_streamwise}
% 	\end{subfigure}
% \caption{Saliva droplet spreading under different exhalation behaviors, as seen from the side, taken at 0.5\,s and 5\,min after the emission.}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/coughing.pdf}
    \caption{Saliva droplet spreading from a coughing source (blue arrow) at (a) $T=1$s and (b) $T=300$s after the emission. The horizontal scale denotes 2\,m social distancing.}
    \label{fig:IEEE_cough_sneez}
\end{figure}

%\todo[inline]{Mythra, please add classroom simulation figure}

%As shown in Fig. \ref{fig:IEEE_cough_sneez}, %and \ref{fig:IEEE_sneez_streamwise},
%the simulation shows the complex particle spreading dynamics when people cough. Even with other people not moving and staying 2\,m (6\,ft) apart, the infectious droplets has swept through the adjacent people within 5 minutes. 
%In the simulation, the static air ventilation openings are working at the flow rate of xxx, which instead of absorbing the fume, helped the fume to permiate through the space slowly and 
%these simulations show the complex particle dynamics when Person A sneezes, and its effect on another Person B at a distance of 2\,m. As seen over a 5 minute time span, gravity causes the larger droplets ($\geq 50\,\mu$m) to quickly fall to the ground where they become significant sources of surface contamination. Whereas the smaller droplets ($\leq 12\,\mu$m) mix with the surrounding air and continue to disperse well past 2\,m, %While the simulation depicts an empty room, community spaces such as classrooms, supermarkets, and restaurants have dynamic environments with more shared spaces,
%increases the potential for transmission. 

The total time of analysis is 5 minutes with non-uniform time steps for both discrete (droplets) and continuous phases (air), to show that the particles can spread over 2\,m of distance, as shown in Fig. \ref{fig:IEEE_cough_sneez}. Since the velocity has been dissipated, the infectious plume will cause continuous exposure to the adjacent people. These results reveal the need for air filtration that can effectively capture the droplets before dispersion.

\subsection{Dosage Criteria}

Realistic data is used to evaluate the risk of a person during the spreading process of the saliva plume of pathogen. Since the saliva is diluted in the air, the virus concentration, measured in PFU/m$^3$ of air, is averaged in a grid-wise manner in the horizontal plane because the particles $P_i$ are discrete objects. Since the robot and people move in a 2-D plane, the 3-D virus concentration can be further averaged vertically for evaluation. The averaging range is the entire room height $H$, in case of possible vertical perturbation of the air. Denote the concentration of virus in saliva as $c$, the averaging grid size as $2l$, the concentration $C$ of virus in the air at time $t$ at grid centered $(x,y)$ is thus generated from the particle distribution $P$ as:
\begin{equation}
    C_P(x,y,t) = \frac{kc}{4Hl^2}\cdot \frac{4\pi}{3} \sum_{P_i(t)\in\{(x-l, x+l)\times(y-l, y+l)\}} r_{P_i}^3,
\end{equation}
where $k$ is the scaling value due to liquid evaporation (hence virus consolidation) in the droplets, and $r_P$ denotes the radius of the particles. Here, we set $c=10^6\, \textnormal{PFU/mL}$ \cite{Schijven2020SARS-CoV2-Concentration} and $k=10$ \cite{aliabadi2010cfd} in the analysis followed.

Since a normal human has a tidal volume of about $V=0.5$L and breathing rate of 12 per minute at rest. Because the tidal volume equivalents to that of a sphere with diameter of 0.1\,m, we set the grid size to be $2l=0.1$m. The ``capture grid" is defined as a grid where an observer stands. The dosage per breathing of the observer is derived from the average particle concentration on the capture grid over 5 seconds. Hence the total dosage the observer receives through an exposure period of $t_e$ (seconds) is obtained:
\begin{equation}
    D_P(x,y)_\textnormal{obs} = \sum_{i=0}^{t_e/5-1}\int_{0}^{5}\frac{ C_P(x,y,5i+t) V}{5}\textnormal{d}t.
    \label{eqn:dosage}
\end{equation}

To increase the robustness of the dosage estimation with respect to location error of the observer, a max dosage $\hat{D}_P(x,y)_\textnormal{obs}$ is taken as the maximum dosage on the 3-by-3 grids centered at $(x,y)$. 
As a reference for severity of exposure, studies of SARS-CoV indicates an at most 5\% chance of developing illness from the virus when exposed under virus dosage of 10\,PFU \cite{Watanabe2010SARS-infectivity}. 
%Assume the observer experiences one exposure to the adjacent cough per half-an-hour, and the threshold dosage within 8 hours of exposure is set at 10 PFU, i.e. the observer at location $(x,y)$ is at risk of infection if $\hat{D}_P(x,y)_{\textnormal{obs}}\geq0.625$, where $t_e=1800$\,s.
Under this criteria, we will build a generalizable model on mobile air filtration in classroom setting in Section \ref{sec:disinfection_sim}.

%\subsection{A Simulation Comparison of Robotic Filtration Versus Stationary Filtration}

%[DO WE STILL NEED THIS PART AS WE ARE RUNNING OVER LENGTH?]

%Under the social distancing guideline, the room with dimensions mentioned above can contain multiple people, as in the case of a classroom. In this case, we place 

%[TODO: PARAMETERIZE THE PATH AND GENERALIZE THE DESIGN PARAMETERS]


%First, we evaluate a case with a single static filter. The static filter operates with the same flow rate as the Bernoulli air filtration module with air flowing through the filter at a rate of 0.047\,$\textnormal{m}^3/\textnormal{s}$ (100 cubic feet per minute). The air filter is simplified as a rectangular prism with size of 0.6\,m $\times$ 0.6\,m $\times$ 1\,m. The filter is placed in the path of the coughing jet at 2\,m from person A. Both the sources cough simultaneously and the spread of virus carrying droplets at different time-steps is shown in Fig. \ref{fig:sim_static}. To compute the concentration of the virus, the space is discretized into cells and the number of droplets per unit area scaled with droplet diameter is used as the concentration of virus. These values are logarithmically scaled for representation in the figures. Indicated by the concentration gradient, the concentration of virus beyond the filter due to person A is 0. However, at time-step 2min, person C is exposed to particles from person D's cough as seen in Fig. \ref{fig:sim_static}b. 

%To explore the static filtration scenario, similar simulation with two static filters each at 2\,m from the source of coughing is shown in Fig. \ref{fig:sim_static_2}. Here both the filters together filter the infectious droplets before they can reach person B and C, thereby eliminating risk of exposure. This shows how strategically placed filtration can significantly reduce transmission and exposure in community settings. However, the expense of static filters per person in community settings becomes quickly impractical. Consider a classroom with $n$ students: this means installing $n$ filters to effectively reduce the risk of transmission.



%NEEDS BETTER EXPLANATION...
%If the coughing jets from them are released simultaneously, the virus dosages at persons B and D, under different air filtration options, are shown in Fig. \ref{}. Specifically, the virus concentration of the entire room at $t=$ is depicted in Fig. \ref{}, corresponding to the period where the virus concentration at Person B is at its maximum. The results show that one static filter at the middle of the room is unable to protect any persons (neither B nor D) from the risk of infection. As a comparison, the air filter on top of the mobile robot is able to keep the dosage at both B and D below the threshold.
%The robot moves in a generalized coverage path to filter the entire room at 0.5\,m/s (Fig. \ref{fig:sim_rob_path}), released from lower left corner of the room at the moment of jet release. After reaching the end of it's path, the robot returns to the start and moves again on the same path. % possibly not necessary... -- Specifically, the peak virus concentration at the middle between the sources is xx and yy, respectively, assuming a virus count of zz/$\mu\textnormal{m}^3$ within the droplets. 
%The robot significantly reduced the risk of exposure to both person B and C by following this specific path since it has absorbed all the emitted particles. % mentioned elsewhere -- This signifies the capability of PCPR as a tool to reduce transmission in closed spaces with multiple people some of who may be infected.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.49\textwidth]{figures/combined_stat3.png}
%    \caption{The concentration of pathogen at (a) t=\,1s and (b) t=2\,min with 2 static filters and (c) t=2\,min with 3 static filters at positions indicated by the magenta '+' mark.}
%    \label{fig:sim_static_2}
%\end{figure}

%Although the robot passes through the first source only briefly after its emission, the robot is also capable of passing through the plume from the second source sometime after the emission, before it spreads through the 6\,ft distance. Actually, literature \cite{aliabadi2010cfd} shows that the plume of saliva droplets looses its velocity within 3 seconds after the emission, and then it mainly follows a slow diffusion process only. Hence, the exact time of emission is not so important for the robot as long as the robot covers the space with its air filter sufficiently taking in the volume of air between neighboring passes. The dynamics of the droplets also proves the feasibility of using robots to clean the indoor air to prevent infection, assuming that people are spaced per recommendation to social distancing (6\,ft or 2\,m), and not moving in the room (i.e. not actively passing and disturbing contaminated areas before they are cleaned by the robot). Although the cleaning factor is merely 5.22\%, the plume of droplets is also sparsely distributed over the workspace, therefore the robot can still achieve high absorption rate as shown in Fig. \ref{fig:sim_robot}.

%\todo[inline]{[Rephrase FIGURES accordingly. Show result with 3 static filters first and then take out the righter-most filter.]}

%As a comparison, we evaluate a case with three static filters spaced equally in the room (at $x=2\,m, 4\,m, 6\,m$, respectively). Each static filter has the same flow rate as the moving filter. Emission of the sources is analogous to the mobile filter case. As shown in Fig. \ref{fig:sim_static_2}c, the three filters together inactivate the infectious droplets before they can reach person B and C, thereby eliminating risk of exposure. This shows how strategically placed filtration can significantly reduce transmission and exposure in community settings. However, the expense of static filters per person in community settings becomes quickly impractical as the space grows.

%What if we do not follow the recommendations from \eqref{efficacy_ratio} and place only 2 static filters in the room? As shown in Fig. \ref{fig:sim_static_2}b, we only set two static filters at $x$ coordinates of 2 and 4, and simulate the same source emission conditions as the mobile filter case. The simulation result shows that 2 minutes after the release, person B is still safe, while person C is exposed to the infectious droplets. The asymmetric arrangement of filters is to show that only when the filters are strategically placed can the healthy persons get proper protection.

%The simple case intuitively showed that making the air filter move is able to clean up infectious bioaerosol faster than a static air filter. This is because bioaerosol particles created from sneezes and coughs are heavier, therefore establishes less diffusion effect. As a result, a mobile filter covering the entire room in a cyclic manner is able to move to infectious plumes actively and clean them within a bounded time after they are created, before they permeate the entire room. The benefit is two-folds: 
%\begin{itemize}
%    \item  Because the cleaning time and spreading region is bounded, there is less chance that other people will be involved in the plume region, and thus poses less chance of infection.
%    \item Since the plume is less spread-out, the volume of air the filter needs to process is smaller, hence a mobile filter achieves faster cleaning rate.
%\end{itemize}

%In Section \ref{sec:disinfection_sim} we will delve into a more complicated and realistic scenatio and evaluate the risk of the ``most vulnerable people" in an emission event under different conditions.
